ALMA Central Molecular Zone Exploration Survey (ACES) I: Overview

The mass flows and energy cycles within the inner regions of galaxies exert a powerful influence on the evolution of the galaxy population. The centre of the Milky Way is the only galactic nucleus for which it is possible to resolve the physical mechanisms that drive these cycles, namely star formation and feedback, while also tracing global (>100 pc) processes which determine where and when star formation and feedback occur. We present an overview of ACES, the 'Atacama Large Millimeter/submillimeter Array (ALMA) CMZ Exploration Survey', a ~1.5" angular resolution, 0.2-3 km/s spectral resolution ALMA Band 3 (85-102 GHz), survey of the 'Central Molecular Zone' (CMZ) -- the inner-100 pc of the Galaxy (l = 359.4 deg to 0.8 deg). ACES spectral setup is tuned to observe optimal tracers of the physical, chemical, and kinematic conditions in over 70 spectral features (e.g. HCO+, HNCO, SiO, H40alpha, complex molecules) of the gas in the CMZ, to derive the properties of all potentially star-forming Galactic Centre gas, from global scales (100 pc) to dense ~0.05 pc structures that are expected to host individual star-forming cores, down to sub-sonic (<0.4 km/s) velocity resolution. In this overview paper, we provide the scientific justification for the ACES survey, explain the choice of observational setup, and describe the data legacy products. Finally, we show some of the initial ACES data which highlight the power of ACES' combination of high angular resolution, unprecedented spatial dynamic range, sensitivity, spectral resolution and spectral bandwidth as an illustration of how ACES aims to understand how global processes set the location, intensity, and timescales for star formation and feedback in the CMZ.

==> tables/linelist.tex <==

\begin{table}
\begin{tabular}{lccc}
\hline\hline
    Line & Rest (GHz) & 12m SPW & References \\
\hline
    HC15N 1-0 & 86.05496 & 25 & Armijos-Abendano et al. (2015) \\
    SO 2(2)-1(1) & 86.09395 & 25 &  \\
    CCS 7(6)-6(5) & 86.1813 & 25 & Armijos-Abendano et al. (2015) \\
    CH3OCH3 2(2,0)-2(1,1) & 86.2267 & 25 & Armijos-Abendano et al. (2015) \\
    SiO 2-1 v=1 maser & 86.24337 & 25 & Stroh et al. (2019) \\
    CH3OCHO 7(3,5)-6(3,4) & 86.2658 & 25 & Armijos-Abendano et al. (2015) \\
    H13CN 1-0 & 86.33992 & 25 & Santa-Maria et al. (2021) \\
    HC(O)NH2 & 86.382755 & 25 &  \\
    HCO 1(0,1)-1(0,0) & 86.6707 & 27 & Armijos-Abendano et al. (2015) \\
    CH3NCO 10(0,10)-9(0,9) & 86.68019 & 27 &  \\
    CH3NCO 10(0,0)-9(0,0) & 86.686556 & 27 &  \\
    HCO 1(0,1)-1(0,0) & 86.7083 & 27 & Armijos-Abendano et al. (2015) \\
    H13CO+ 1-0 & 86.7543 & 27 & Santa-Maria et al. (2021) \\
    HCO 1(0,1)-1(0,0) & 86.7774 & 27 & Armijos-Abendano et al. (2015) \\
    HCO 1(0,1)-1(0,0) & 86.8057 & 27 & Armijos-Abendano et al. (2015) \\
    C2H5CN & 86.819845 & 27 &  \\
    CH3CH2CN & 86.81984 & 27 &  \\
    SiO 2-1 & 86.84696 & 27 & Santa-Maria et al. (2021) \\
    HC17O+ (1-0) & 87.0575347 & 27 &  \\
    HN13C 1-0 & 87.09085 & 27 &  \\
    HNCO 4-3 & 87.925238 & 31 & Kuan \& Snyder (1996) \\
    HCO+ 1-0 & 89.18852 & 29 & Santa-Maria et al (2021) \\
    SO2 7(3,5)–8(2,6) & 97.70234 & 33 & Jones et al. (2008) \\
    34SO 3(2)–2(1) & 97.7154 & 33 & Jones et al. (2008) \\
    CH3CONH2 & 97.810915 & 33 &  \\
    HCOCH2OH & 97.9196993 & 33 &  \\
    CS 2-1 & 97.98095 & 33 &  \\
    CH3CH2CN 11(2,10)–10(2,9) & 98.17757 & 33 & Jones et al. (2008) \\
    CH3OCHO  8(7,1)–7(7,0) E & 98.18219 & 33 & Jones et al. (2008) \\
    CH$_3$(18)OH & 98.206527 & 33 &  \\
    33SO 3(2)-2(1) & 98.483155 & 33 &  \\
    HC5N & 98.512524 & 33 &  \\
    CH3CHO 5(1,4)–4(1,3) A– & 98.90095 & 33 & Jones et al. (2008) \\
    H40 Alpha & 99.02295 & 33 &  \\
    CH3NH2 & 99.1272454 & 33 &  \\
    CH3C3N & 99.1502601 & 33 &  \\
    H50 Beta & 99.22521 & 33 &  \\
    SO 3(2)-2(1) & 99.29987 & 33 &  \\
    HCCNC & 99.35425 & 33 &  \\
    CH3C(13)CH 6-5 & 99.46377 & 33 &  \\
    HC13CCN 11-10 & 99.65184 & 35 & Jones et al. (2008) \\
    HCC13CN 11-10 & 99.66147 & 35 & Jones et al. (2008) \\
    CH3CH2CN  11(2,9)–10(2,8) & 99.68151 & 35 & Jones et al. (2008) \\
    (13)CH3CCH 6-5 & 99.75655 & 35 &  \\
    S18O & 99.803794 & 35 &  \\
    SO 4(5)-4(4) & 100.02956 & 35 & Jones et al. (2008) \\
    HC3N 11-10 & 100.0763 & 35 &  \\
    H2CCO & 100.094514 & 35 &  \\
    NS+ & 100.198 & 35 &  \\
    HC3N 11-10 v6=1 & 100.240584 & 35 &  \\
    HC3N 11-10 v7=1 & 100.32241 & 35 & Jones et al. (2008) \\
    CH3OCH3 6(2,5)–6(1,6) EA+AE & 100.460412 & 35 & Jones et al. (2008) \\
    CH3OCH3 6(2,5)–6(1,6) EE & 100.463066 & 35 & Jones et al. (2008) \\
    CH3OCH3 6(2,5)–6(1,6) AA & 100.465708 & 35 & Jones et al. (2008) \\
    HC3N 11-10 v7=1 & 100.466174 & 35 &  \\
    CH3NC & 100.524249 & 35 &  \\
    H2CCN & 100.5980668 & 35 &  \\
    CH3CH2CN  11(1,10)–10(1,9) & 100.614291 & 35 & Jones et al. (2008) \\
    NH2CN 5(1,4)-4(1,3) & 100.6295 & 35 & Jones et al. (2008) \\
    CH3OH & 100.638872 & 35 &  \\
    HC3N 11-10 v7=2 & 100.708784 & 35 & Jones et al. (2008) \\
    HC3N 11-10 v7=2 & 100.711064 & 35 & Jones et al. (2008) \\
    HC3N 11-10 v7=2 & 100.714395 & 35 & Jones et al. (2008) \\
    SO2 2(2,0)-3(1,3) & 100.878105 & 35 & Jones et al. (2008) \\
    C2H5OH & 100.9901131 & 35 &  \\
    CH2CHO  5(2,4)–4(2,3) & 101.024438 & 35 & Jones et al. (2008) \\
    CH3SH 4(-1)–3(-1) E & 101.02975 & 35 & Jones et al. (2008) \\
    CH3SH  4(0)–3(0) A & 101.13916 & 35 & Jones et al. (2008) \\
    CH3SH  4(0)–3(0) E & 101.13965 & 35 & Jones et al. (2008) \\
    H2C(34)S & 101.2843139 & 35 &  \\
    H2CO  6(1,5)–6(1,6) & 101.332987 & 35 & Jones et al. (2008) \\
\hline\hline
\end{tabular}
\end{table}


==> tables/linelist2.tex <==

\begin{longtable}{lccc}
\caption{Molecular line transitions, rest frequencies, spectral windows (SPWs) in the 12-m array configuration, and references.\label{tab:lines}} \\
\toprule
    Line & Rest (GHz) & 12m SPW & References \\
\midrule
\endfirsthead

\toprule
    Line & Rest (GHz) & 12m SPW & References \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot

HC15N 1-0 & 86.05496 & 25 & Armijos-Abendano et al. (2015) \\

SO 2(2)-1(1) & 86.09395 & 25 &  \\
CCS 7(6)-6(5) & 86.1813 & 25 & Armijos-Abendano et al. (2015) \\
CH3OCH3 2(2,0)-2(1,1) & 86.2267 & 25 & Armijos-Abendano et al. (2015) \\
SiO 2-1 v=1 maser & 86.24337 & 25 & Stroh et al. (2019) \\
CH3OCHO 7(3,5)-6(3,4) & 86.2658 & 25 & Armijos-Abendano et al. (2015) \\
H13CN 1-0 & 86.33992 & 25 & Santa-Maria et al. (2021) \\
HC(O)NH2 & 86.382755 & 25 &  \\
HCO 1(0,1)-1(0,0) & 86.6707 & 27 & Armijos-Abendano et al. (2015) \\
CH3NCO 10(0,10)-9(0,9) & 86.68019 & 27 &  \\
CH3NCO 10(0,0)-9(0,0) & 86.686556 & 27 &  \\
HCO 1(0,1)-1(0,0) & 86.7083 & 27 & Armijos-Abendano et al. (2015) \\
H13CO+ 1-0 & 86.7543 & 27 & Santa-Maria et al. (2021) \\
HCO 1(0,1)-1(0,0) & 86.7774 & 27 & Armijos-Abendano et al. (2015) \\
HCO 1(0,1)-1(0,0) & 86.8057 & 27 & Armijos-Abendano et al. (2015) \\
C2H5CN & 86.819845 & 27 &  \\
CH3CH2CN & 86.81984 & 27 &  \\
SiO 2-1 & 86.84696 & 27 & Santa-Maria et al. (2021) \\
HC17O+ (1-0) & 87.0575347 & 27 &  \\
HN13C 1-0 & 87.09085 & 27 &  \\
HNCO 4-3 & 87.925238 & 31 & Kuan \& Snyder (1996) \\
HCO+ 1-0 & 89.18852 & 29 & Santa-Maria et al (2021) \\
SO2 7(3,5)–8(2,6) & 97.70234 & 33 & Jones et al. (2008) \\
34SO 3(2)–2(1) & 97.7154 & 33 & Jones et al. (2008) \\
CH3CONH2 & 97.810915 & 33 &  \\
HCOCH2OH & 97.9196993 & 33 &  \\
CS 2-1 & 97.98095 & 33 &  \\
CH3CH2CN 11(2,10)–10(2,9) & 98.17757 & 33 & Jones et al. (2008) \\
CH3OCHO  8(7,1)–7(7,0) E & 98.18219 & 33 & Jones et al. (2008) \\
CH$_3$(18)OH & 98.206527 & 33 &  \\
33SO 3(2)-2(1) & 98.483155 & 33 &  \\
HC5N & 98.512524 & 33 &  \\
CH3CHO 5(1,4)–4(1,3) A– & 98.90095 & 33 & Jones et al. (2008) \\
H40 Alpha & 99.02295 & 33 &  \\
CH3NH2 & 99.1272454 & 33 &  \\
CH3C3N & 99.1502601 & 33 &  \\
H50 Beta & 99.22521 & 33 &  \\
SO 3(2)-2(1) & 99.29987 & 33 &  \\
HCCNC & 99.35425 & 33 &  \\
CH3C(13)CH 6-5 & 99.46377 & 33 &  \\
HC13CCN 11-10 & 99.65184 & 35 & Jones et al. (2008) \\
HCC13CN 11-10 & 99.66147 & 35 & Jones et al. (2008) \\
CH3CH2CN  11(2,9)–10(2,8) & 99.68151 & 35 & Jones et al. (2008) \\
(13)CH3CCH 6-5 & 99.75655 & 35 &  \\
S18O & 99.803794 & 35 &  \\
SO 4(5)-4(4) & 100.02956 & 35 & Jones et al. (2008) \\
HC3N 11-10 & 100.0763 & 35 &  \\
H2CCO & 100.094514 & 35 &  \\
NS+ & 100.198 & 35 &  \\
HC3N 11-10 v6=1 & 100.240584 & 35 &  \\
HC3N 11-10 v7=1 & 100.32241 & 35 & Jones et al. (2008) \\
CH3OCH3 6(2,5)–6(1,6) EA+AE & 100.460412 & 35 & Jones et al. (2008) \\
CH3OCH3 6(2,5)–6(1,6) EE & 100.463066 & 35 & Jones et al. (2008) \\
CH3OCH3 6(2,5)–6(1,6) AA & 100.465708 & 35 & Jones et al. (2008) \\
HC3N 11-10 v7=1 & 100.466174 & 35 &  \\
CH3NC & 100.524249 & 35 &  \\
H2CCN & 100.5980668 & 35 &  \\
CH3CH2CN  11(1,10)–10(1,9) & 100.614291 & 35 & Jones et al. (2008) \\
NH2CN 5(1,4)-4(1,3) & 100.6295 & 35 & Jones et al. (2008) \\
CH3OH & 100.638872 & 35 &  \\
HC3N 11-10 v7=2 & 100.708784 & 35 & Jones et al. (2008) \\
HC3N 11-10 v7=2 & 100.711064 & 35 & Jones et al. (2008) \\
HC3N 11-10 v7=2 & 100.714395 & 35 & Jones et al. (2008) \\
SO2 2(2,0)-3(1,3) & 100.878105 & 35 & Jones et al. (2008) \\
C2H5OH & 100.9901131 & 35 &  \\
CH2CO  5(2,4)–4(2,3) & 101.024438 & 35 & Jones et al. (2008) \\
CH3SH 4(-1)–3(-1) E & 101.02975 & 35 & Jones et al. (2008) \\
CH3SH  4(0)–3(0) A & 101.13916 & 35 & Jones et al. (2008) \\
CH3SH  4(0)–3(0) E & 101.13965 & 35 & Jones et al. (2008) \\
H2C(34)S & 101.2843139 & 35 &  \\
H2CO  6(1,5)–6(1,6) & 101.332987 & 35 & Jones et al. (2008) \\

\end{longtable}

